Grounding Open-Domain Instructions to Automate Web Support Tasks

Grounding natural language instructions on the web to perform previously unseen tasks enables accessibility and automation. We introduce a task and dataset to train AI agents from open-domain, step-by-step instructions originally written for people. We build RUSS (Rapid Universal Support Service) to tackle this problem. RUSS consists of two models: First, a BERT-LSTM with pointers parses instructions to ThingTalk, a domain-specific language we design for grounding natural language on the web. Then, a grounding model retrieves the unique IDs of any webpage elements requested in ThingTalk. RUSS may interact with the user through a dialogue (e.g. ask for an address) or execute a web operation (e.g. click a button) inside the web runtime. To augment training, we synthesize natural language instructions mapped to ThingTalk. Our dataset consists of 80 different customer service problems from help websites, with a total of 741 step-by-step instructions and their corresponding actions. RUSS achieves 76.7% end-to-end accuracy predicting agent actions from single instructions. It outperforms state-of-the-art models that directly map instructions to actions without ThingTalk. Our user study shows that RUSS is preferred by actual users over web navigation.

==> byemath.tex <==

\subsection{Problem Formulation}

\TODO{is there anything here that was not said above?}

For a webpage $w =((e_s, attr_s))_{s=1:C}$ with $C$ elements, $attr_s$ is the dictionary mapping each web attribute of $e_s$ to its value. We let $W = w_{1:n} = (w_1, ...,w_n)$ be the sequence of webpages at the start of instructions $1
:n$ and similarly  $V = v_{1:n} = (v_1, ...,v_n)$ where $v_m =((n_s, v_s))_{s=1:r}$ the sequence of variables available to the agent at each instruction $1:n$. 

The transition function for $W$ and $V$ is defined as: 
\begin{align*}
    (w_m, v_m) &= \phi(a_{m-1}, w_{m-1}, v_{m-1})
\end{align*}
$a_m$ is the action tuple, $(\alpha_m, e_m, p_m)$, where $\alpha_m$ is the operation, $e_m$ is the element, and $p_m$ is the optional variable parameter. It follows: 

\begin{equation*}
    (w_{m}, v_{m}) = \phi(\alpha_{m-1}, e_{m-1}, p_{m-1}, w_{m-1}, v_{m-1})
\end{equation*}

Given a sequence of instructions $S = (i_1, \ldots, i_n)$, where $i_m$ is the $m^{th}$ natural-language instruction in the set, our task is to generate a web agent that predicts and executes $A=(a_1, \ldots, a_n)$, the corresponding sequence of action tuples on $W = (w_1, ...,w_n)$, the webpages. 

An instruction set $S$ will contain more than one instruction $i_m$ that are to be executed sequentially.  The probability of generating a the correct sequence of actions for a given the instruction set, starting webpage, and transition function is therefore given as: 

\begin{equation*}
    p(a_{1:n} | i_{1:n}, w_1, v_1, \phi) = \\ 
    {\displaystyle \prod_{i=1}^{n} p(a_i | i_{1:i}, a_{1:i-1}, w_1, v_1, \phi )}
\end{equation*}

At the beginning of each instruction set, there are no stored variables and $v_1 = ()$. Crucially, instructions within the same set are considered independent of each other (prior instructions do not determine how later instructions are interpreted). This allows us to perform evaluation of our model on a per instruction basis. The transition $\phi$ is used to derive $W$ and $V$ as $(w_{i-1}, v_{i-1} = \phi(a_{i-2}, \phi(a_{i-3}, \phi (...))) $: 

\begin{equation*}
    p(a_{1:n} | i_{1:n, w_1, \phi}) = {\displaystyle \prod_{i=1}^{n} p(a_i | i_{i}, w_{i-1}, v_{i-1} )}
\end{equation*}

To allow  semantic parsing to an intermediate representation of the natural language instructions, we can decompose $p(a_i | i_{i}, w_{i-1}, v_{i-1} )$ as: 

\begin{align*}
    p(a_i | i_{i}, w_{i}, v_{i} ) = &{\displaystyle \sum_{E}^{} p(a_i | \epsilon, i_{i}, w_{i}, v_{i})} * \\
    &  p(\epsilon | i_{i}, w_{i}, v_{i}) = \\ 
     &{\displaystyle \sum_{E}^{} p(a_i | \epsilon_i, w_{i-1})} *\\ &  p(\epsilon_i | i_{i}, w_{i}, v_{i})
\end{align*}

Here $\epsilon$ is an expression in WebLang and $E_i$ is the set of all possible WebLang expressions that maps to $\alpha_i$ and $p_i$. $a_i = (\alpha_i, e_i, p_i)$, and $\epsilon_i$ determines $\alpha_i$ and $p_i$ so: 
Let $\hat{\epsilon_i}$ be the most likely WebLang expression for $i_i$ that grounds to $\alpha_i, p_i, e_i$, then: 
\begin{align*}
    p(a_i | i_{i}, w_{i-1}, v_{i-1} ) \approx &p(a_i | \hat{\epsilon}, w_{i}) * \\
    &p(\hat{\epsilon} | i_{i})
\end{align*}

The effect of Equation xyz is to ground the natural language instruction $i_i$ on the webpage $w_{i}$ and the variables $v_{i}$.  $p(e_i | \hat{\epsilon_i}, w_{i})$ defines the webpage element (if any) recovered for $\hat{\epsilon_i}$ WebLang parse, and $p(\hat{\epsilon} | i_{i}, w_{i}, v_{i})$ defines the WebLang parse of the given natural langague instruction $i_i$. \RUSS trains a universal \text{\bf Parsing Model} which optimizes $p(\hat{\epsilon} | i_{i}, w_{i}, v_{i})$ and the \text{\bf Grounding Model} maximizes $p(a_i | \hat{\epsilon_i}, w_{i})$, which is equivalent to resolving @webagent.retrieve given the WebLang. This 2-part hybrid architecture of \RUSS allows it to master new tasks on-the-job from open-domain natural language instructions by identifying action tuples that maximize $p(a_i | i_{i}, w_{i}, v_{i} )$ . Finally the transition function $\phi$ is the \textbf{Runtime} that determines how WebLang functions are executed in realtime by \RUSS. 

==> task.tex <==

\begin{table*}[h]
\small
\centering
\begin{tabular}{p{5.3cm}|p{9cm}}
\toprule
\textbf{Agent Action} & \textbf{Description} \\
\midrule
@goto(\textit{url}) & Navigate to the given URL \\ 
\hline
@enter(\textit{element\_id}, \textit{dict\_key}) & Find the closest match to the given dictionary key and enter its value in the given input element\\
\hline
@click(\textit{element\_id}) & Click on the given element \\ 
\hline
@read(\textit{element\_id}) & Read the content of the given element to the user \\ 
\hline
@say(\textit{message}) & Read the given message to the user \\
\hline
@ask(\textit{dict\_key}) & Ask the user for the value of a dictionary key \\
\bottomrule
\toprule
\textbf{Grounding Function} & \textbf{Description} \\
\midrule
\text{@retrieve}(\textit{descr}, \textit{type}, \textit{loc}, \textit{above}, \textit{below}, \textit{right\_of}, \textit{left\_of}) : \textit{element\_id} & Retrieves the elements matching the descriptors, returns an \textit{element\_id}.\\
\bottomrule
\end{tabular}
\caption{WebLang Agent Actions and a Grounding Function}
\label{tab:weblang}
\end{table*}

\section{Task}
%We frame the tasks as commonly presented in the real world. 
Given a set of natural language instructions  $S = (i_1, \ldots, i_n)$ and a starting web page, our task is to construct an agent that follows the instructions through a series of action $A=(a_1, \ldots, a_n)$. Actions include web navigation and end-user interaction in order to obtain necessary information. 
Surveying online customer service tasks, $6$ action operations were identified as necessary for agents: open a URL page, enter text, click on buttons, say something to the user, read the results to the user, and ask user for some information. Details  are described in Table~\ref{tab:weblang}, where elements on a web page are assumed to be given unique element IDs. 

%combined with previous paragraph to avoid duplication and reduce length:
%Given a sequence of instructions $S = (i_1, \ldots, i_n)$, %where $i_m$ is the $m^{\text{th}}$ natural-language instruction in the sequence, 
%our goal is to generate the corresponding series of actions $A=(a_1, \ldots, a_n)$, whose semantics are given in Table~\ref{tab:weblang}.

In natural language instructions, however, the elements that the agent has to interact with such as buttons are described based on their visual appearance when rendered and not their html IDs.  For instance, the instruction may read ``fill out the textbox under Apply Gift''. Such descriptions must be grounded to specific element IDs on the page.  Previous work uses an end-to-end neural network to return an element ID from natural language commands and given webpages~\cite{phrasenode}.  
We propose a two step approach. %- there's no description of anything hybrid following, it's a sequence not a hybrid

We first capture the semantics of the natural language description at a high level, independent of any webpage, then use the formal representation to identify the specific element on a given web page.  To achieve this, we propose WebLang, a novel domain-specific language whose primitives include the 6 {\em agent actions} and a {\em grounding function} @retrieve. @retrieve maps a formal description of an element to an element\_id on the webpage, that can be used in agent actions. 

\RUSS the $S$:
\begin{enumerate}
\itemsep-0.3em 
\item Semantic Parser.   Maps open-domain natural language instruction to its WebLang parse.   
\item Grounding model.  Maps @retrieve functions in the WebLang parse to the  elements on a given web page; the result is a {\em grounded} WebLang program, comprising a sequence of agent actions operating on disambiguated elements. 
\item A Runtime.  Executes the agent actions by performing the web operations in an automated browser while interacting with the user.% over voice - let's not randomly add voice here for the first time
\end{enumerate}




